An explanatory evo-devo model for the developmental hourglass

The "developmental hourglass" describes a pattern of increasing morphological divergence towards earlier and later embryonic development, separated by a period of significant conservation across distant species (the "phylotypic stage"). Recent studies have found evidence in support of the hourglass effect at the genomic level. For instance, the phylotypic stage expresses the oldest and most conserved transcriptomes. However, the regulatory mechanism that causes the hourglass pattern remains an open question. Here, we use an evolutionary model of regulatory gene interactions during development to identify the conditions under which the hourglass effect can emerge in a general setting. The model focuses on the hierarchical gene regulatory network that controls the developmental process, and on the evolution of a population under random perturbations in the structure of that network. The model predicts, under fairly general assumptions, the emergence of an hourglass pattern in the structure of a temporal representation of the underlying gene regulatory network. The evolutionary age of the corresponding genes also follows an hourglass pattern, with the oldest genes concentrated at the hourglass waist. The key behind the hourglass effect is that developmental regulators should have an increasingly specific function as development progresses. Analysis of developmental gene expression profiles from Drosophila melanogaster and Arabidopsis thaliana provide consistent results with our theoretical predictions.

==> tex_files/discussion-long.tex <==

\vspace{0.1in}
\noindent {\bf Discussion}\\
The pattern of conservation during early development has been a longstanding, 
ongoing debate in developmental biology. In the past, this debate has mostly 
been approached with comparative studies of morphological and phenotypic 
similarities between different species \cite{richardson1997there, richardson2002haeckel, von1828entwicklungsgeschichte}. 

More recently, the focus has shifted towards such studies at the genomic 
and molecular level \cite{domazet2010phylogenetically, irie2007vertebrate, 
kalinka2010gene, piasecka2013hourglass, quint2012transcriptomic}. These studies investigate conservation of 
gene expression variation, sequence conservation, selective constraint on coding 
sequences, and evolutionary ``age'' of genes.  These genomic studies further 
revealed several contradicting observations: some studies support strong conservation 
in earlier developmental stages \cite{rasmussen1987new, roux2008developmental, piasecka2013hourglass} while others report strongest conservation 
in the mid-developmental stage \cite{irie2011comparative, irie2007vertebrate, kalinka2010gene, levin2012developmental, 
quint2012transcriptomic, hazkani2005search, domazet2010phylogenetically, irie2011comparative, galis2001testing, 
cruickshank2008microevolutionary, galis2001testing, levin2012developmental}. 
Nevertheless, the pattern of hourglass, observed 
from highly divergent species across deep phylogenetic scales, including fish, flies and plant, 
suggest that the observed patterns of conservation may stem from fundamental principles that may drive developmental processes.  

However, what these principles are, and why developmental progressions follow hourglass patterns, 
remain unresolved.  Consequently, the principles that govern the evolution of these developmental 
processes are elusive to experimental analyses.  On the one hand, earlier stages may be conserved 
because changes in earlier developmental stages will have large cascading effects in later 
developmental stages \cite{riedl1978order, arthur1984mechanisms, rasmussen1987new}.  This model is often cited as a 
support for the funnel-like pattern of development.  On the other hand, later stages may experience 
less constraint because as development progresses, gene interactions become more modular, and 
perturbations only affect localized modules rather than the whole organisms \cite{raff1996shape}.  
These distinctive schools of thoughts, which we will refer to as the ``temporal'' constraint model
 and the ``spatial'' constraint model respectively following Tian et al. \cite{tian2013dictyostelium}, 
are both appealing.  The temporal constraint model is intuitive in that any perturbations in the 
earlier developmental stages are likely to have amplified deleterious effects in later stages.  
The spatial model is biologically highly relevant as the modularized biological structures as an 
outcome of developmental processes are widespread in the tree of life.

In fact, it should be noted that it is not necessarily clear that these two models should reach 
contrasting patterns of development (funnel-like versus hourglass).  A main difficulty in evaluating 
these models is a lack of explicit underlying mechanisms that drive evolution of developmental processes.  
In this study, we developed an evolutionary model of development that combines fundamental aspects 
of both models: large effects of perturbations in early interactions, and high modularity of later 
developmental stages.  A key component of this model is the idea that genes that function in early 
development are more ‘general’ compared to those who function in later developmental stages.  This is 
based on the idea that genes in early developmental stages are likely to function as building blocks 
of developmental patterns, and as such may affect multiple different processes downstream.  A flip 
side of this idea is that as development progresses, gene interactions become more modular, and the 
functional role of each gene becomes more ‘specific’.  Genes expressed in later developmental stages 
may encode functions that are specific with respect to temporal and spatial confinements, rather than 
affecting basic developmental scaffolds. 

Based upon these ideas, we built simple models of functional gene interactions during developmental 
progression.  Specifically, we introduce the concept of the developmental gene execution network, 
which is composed of genes that change their functional states throughout development to execute the 
developmental program.  Genes change functional states to give rise to more specialized cells and the 
development progresses. Our model captures the execution of this program during development in the form of 
a network of transitioning genes. We also captured how this network, referred to as the DGEN of the organism, 
evolves over time. Our evolutionary scheme involves a simple constraint that for a final development to be 
successful, a certain number of genes need to be present in the final stage. This is based upon the idea that 
there may exist a minimal gene set that is required for a successful completion of developmental processes. 
Individuals that fail to meet this basic criterion are removed from the whole population, in a process 
similar to a simple truncation selection scheme.  

We thus explored how these processes (executed by networks) have evolved over time and exhibit specific patterns. 
Remarkably, we show that under these simple assumptions, the resulting gene execution network takes a shape of 
``hourglass'' in which mid-developmental stage harbors fewest number of gene components compared to early and 
late developmental stages.  The outcome of developmental hourglass is robust under a variety of parameter combinations.  
Thus our model provides potential underlying genetic mechanisms for the observed genome-wide patterns of developmental constraints.  

Moreover, we tested several aspects of developmental gene execution networks in light of genomic studies of 
developmental hourglass.  We show that mutations or other perturbations close to the waist have the most lethal 
effect on the development of the organism. The ‘age’ of genes also follow the hourglass pattern so that genes 
in the waist of hourglass are the most evolutionarily old.  These patterns are consistently observed for a wide 
range of parameters. The conservation patterns in other properties such as developmental constraints or the patterns 
of similarity uncovered in comparative studies may be consequences of the underlying developmental hourglass.  

In this study we have focused on the development of an abstract model, and examine concordance between the model 
and data using developmental transcriptome profiles of fruitflies.  IIn the future studies, it may be possible to 
infer the actual underlying DGEN of model organisms.  For example, much information on gene regulatory networks of 
sea urchin is available (refs).  These data in principle would allow us to identify functionally transitioning genes 
in certain developmental stages.  We could then directly test our hypothesis that the functionally transitioning genes 
(and gene interactions) that appear to be most critical at or near the waist of the DGEN hourglass. 

The hourglass effect (or sometimes referred to as the bowtie effect for a similar looking structure) 
has also been observed in other complex natural and technological systems that exhibit hierarchical 
modularity in their structure and are subject to evolution \cite{beutler2004inferences, 
csete2004bow, doyle2011architecture, tieri2010network,  zhao2006hierarchical}. 
A famous technological 
system that is structured as an hourglass is the Internet protocol stack \cite{akhshabi2013evolution}. In that system, nodes 
are communication protocols and links represent services. In \cite{akhshabi2013evolution}, we proposed EvoArch, an abstract 
model to study the evolution of protocol stacks. EvoArch predicts that protocol stacks evolve to shape 
like an hourglass under a wide range of experimental scenarios. There are several uncanny similarities 
between EvoArch and the developmental hourglass explored in the current study.  For example a protocol 
stack is a layered network similar to a DGEN: as we move up the protocol stack, communication protocols 
become more application-specific and the network gradually becomes sparser.  Moreover, the waist of 
the hourglass corresponds to the most critical and oldest protocols. 
In the EvoArch model, the intrinsic competition between protocols that offer similar services shapes 
the network over time to look like an hourglass. In a similar context, the genomic program that is 
executed during development uses genes for genetic computation to drive the process towards successful 
development. Gene regulation is costly and so an implicit competition between genes for regulation and 
transmission of genetic information during development is an interesting viewpoint on how embryonic 
development works at evolutionary time scales. Evolution may function to optimize this program and 
use as few genes as possible to perform the same genetic computation while keeping the system robust 
to perturbations. 
Consequently, EvoArch can be an interesting model even in the context of embryonic 
development. In the future, we plan to study embryonic development, and in general the evolution of 
hierarchical modular networks in an optimization framework. Such an approach can provide more direct 
insight into the several biological processes.



%The funnel-like versus hourglass model of conservation 
%is an ungoing debate in developmental biology. 
%In the past, this debate has mostly been approached with comparative 
%studies of morphological and phenotypic similarities between 
%different species \cite{richardson1997there, richardson2002haeckel, von1828entwicklungsgeschichte}.
%More recently, the focus has shifted towards such studies 
%at the genomic and molecular level \cite{domazet2010phylogenetically, irie2007vertebrate, 
%kalinka2010gene, piasecka2013hourglass, quint2012transcriptomic}.
%However, there have been several contradicting observations over the years.

%A main issue in previous comparative studies is the definition and identification of 
%the phylotypic stage in different species. The term 
%phylotypic stage has been used in many different contexts and it is not exactly clear 
%what constitutes this stage. Phylotypic stage has been used to refer to the stage of 
%maximum similarity between different species in terms of several different properties such as 
%morphological, molecular, and genetic patterns during development, or the processes 
%driving it \cite{}.
%On the other hand, different species evolve in different environments 
%and are subject to different evolutionary pressure. 
%So even if we have a clear definition of the phylotypic stage, 
%that stage can be different in terms of developmental time, 
%duration, shape, or even the underlying developmental 
%processes for different species. This would complicate the 
%applicability of comparative studies in identifying the phylotypic stage 
%or the conservation pattern during development.

%In this paper, we focused on the execution of developmental 
%process at the genomic level and the corresponding evolutionary 
%mechanisms that can act to change these processes.
%The GRN of an organism encodes the genomic program that 
%is executed during development. This program starts with the 
%regulatory states of the maternal genes as its initial configuration 
%and then proceeds in a semi-autonomous fashion afterwards. Genes change functional 
%states to give rise to more specialized cells and the embryo gradually 
%develops while the various different tissues of the organism take shape.
%We presented a model to capture the execution of this  
%program during development in the form of a network of unfolding 
%regulatory dependencies between transitioning genes in time and space.
%We also captured how this network, referred to as the DGDN of the organism,
%evolves over time.
%Using this model, we predict that the hourglass pattern is a fundamental 
%property of development for any organism and emerges in the number of transitioning genes
%as long as the underlying evo-devo dynamics follow a set of general rules:
%1) During development, the specificity of the 
%developmental stages should increase over time and 
%the DGDN should become sparser. 2) At the evolutionary 
%scale, the mechanisms that change the DGDN of the organism
%and in particular, the neomorphic-mutations (NM) events, 
%and the potential regulatory failures (RFs) 
%and developmental failures (DFs) that follow them,
%should satisfy certain conditions that preserve the structure 
%of the DGDN (See Section Model Description). Under these 
%conditions, the shape of the resulting DGDNs follow the hourglass 
%pattern: the number of transitioning 
%genes decreases until the waist and then increases until 
%reaching the last stage of embryonic development. 
%Furthermore, mutations or any perturbation close to 
%the waist have the most lethal effect on the development of the organism.
%The lethality of these mutations mirrors the hourglass structure 
%and as a result, the age and the prevalence of genes also 
%follow the hourglass pattern for a wide range of parameters. 

%Our model predicts that the hourglass pattern emerges 
%as a result of some simple but general laws that govern the 
%evolution of embryonic development and the processes that drive it. 
%These laws are not tied to any specific organism and so 
%a similar pattern should emerge in any organism that is subject to these laws.
%As a result, if one is able 
%to define developmentally equivalent stages or processes 
%between distinct species for the purpose of comparative studies, 
%then we can expect to find similarities at different levels
%between these species. However, we believe 
%that the root cause of the previous 
%observations in comparative studies is the 
%underlying hourglass pattern in transitioning genes during development. 
%The conservation pattern in other properties such 
%as developmental constraints or the patterns of similarity uncovered
%in comparative studies are a consequence of 
%this fundamental emergent evolutionary phenomena.


%Our model works under the assumption that the specificity of developmental stages increases
%as the various spatial domains of the embryo gradually take shape. The increasing specificity 
%manifests itself in several different developmental properties.
%One expects that the active functionalities of transitioning genes become more specific to the 
%the corresponding spatial domains and so more tissue-specific. A related observation 
%has been made in \cite{}. Also, due to the gradual separation of the spatial domains during development,
%the cost of cross-domain intercellular signaling increases \cite{}. As a result, the DGDNs become 
%sparser as we move downstream. This pattern of increasing specificity is also observed 
%at the cellular level taking place through the repetitive process of cell differentiation and specialization which 
%gives rise to the various tissues in the organism \cite{}. The increasing specificity seems
%to be an intrinsic property of the development and is required in our model for the emergence of 
%the hourglass pattern.

%Under the increasing specificity assumption, our model predicts the existence of a phylotypic stage.
%This stage includes the most critical 
%transitioning genes during development. Mis-regulation of these genes 
%has the most lethal effect on the developing embryo. These observations are in 
%agreement with previous studies which have shown that genes expressed during the phylotypic stage 
%are the most developmentally constrained \cite{}. Furthermore, our model shows that these 
%genes can be the oldest and most prevalent genes in the population. The hourglass pattern 
%underlying the age of genes \cite{domazet2010phylogenetically, quint2012transcriptomic} and the sequence conservation \cite{kalinka2010gene, quint2012transcriptomic, irie2007vertebrate} have been observed in previous studies.
%However, some of these findings have been questioned. Our model predicts that such a pattern arises 
%from the set of regulatory genes whose functional state transitions drives the developmental
%process. 

%The GRN of an organism encodes the genomic program that 
%is executed during development. This program 
%is represented in the form of regulatory relations between 
%the genes of that organism as well as the functional
%rules that determine the exact regulatory states of each 
%gene from its inputs. The genomic program starts with the 
%regulatory states of the maternal genes as its initial configuration 
%and then proceeds in a semi-autonomous fashion afterwards. Genes change functional 
%states to give rise to more specialized cells and the embryo gradually 
%develops while the various different tissues of the organism take shape.
%Our model captures the execution of this genomic program with the developmental gene regulatory network (DGDN).
%A DGDN is an abstract representation of a dynamic process as it unfolds over time and space.
%It does not attempt to capture the execution of the GRN of a specific organism. However,
%a DGDN can be extended to become more organism-specific by adding more information 
%to the nodes, i.e., the transitioning genes as well the functional rules that determine the 
%state of each genes at each stage of the development. In such a case, we expect that more 
%organism-specific insight can be gained from our model. 
%This is an interesting direction for future work.

%The hourglass effect (or sometimes referred to 
%as the bowtie effect for a similar looking structure) has also 
%been observed in other complex natural and technological 
%systems that exhibit hierarchical modularity in their
%structure and are subject to evolution \cite{beutler2004inferences, csete2004bow, doyle2011architecture, tieri2010network,  zhao2006hierarchical}.
%A famous technological system that is structured as an hourglass 
%is the Internet protocol stack \cite{saamer-evoarch:11}. 
%In that system, nodes are communication protocols and links represent 
%services. In \cite{saamer-evoarch:11}, we proposed EvoArch, an abstract model to study the evolution of protocol stacks.
%EvoArch predicts that protocol stacks evolve to shape like an hourglass under a wide range of 
%experimental scenarios. Furthermore, the waist of the hourglass corresponds to the most critical and oldest 
%protocols. EvoArch has several similar aspects as the model presented in this paper.
%A protocol stack is a layered network similar to a DGDN and the goal of the system 
%is to provide a set of Internet applications from a set of elementary technological inputs.
%As we move up the protocol stack, communication protocols become more application-specific and the network gradually
%becomes sparser.
%In that model, the intrinsic competition between protocols that offer similar services
%shapes the network over time to look like an hourglass. This competition is imposed 
%on the system to optimize its performance under technological constraints set by the 
%environment the system evolves in. In a similar context, the genomic program that is executed 
%during development, uses genes for genetic computation to drive the process towards its final form. 
%Gene regulation is costly and so an implicit competition between genes for regulation and transmission of genetic information 
%during development is an interesting viewpoint on how embryonic development works at evolutionary
%time scales. 
%Evolution then acts to optimize this program and use as few genes as possible to 
%perform the same genetic computation while keeping the system robust to perturbations.
%In that view, EvoArch can be an interesting model even in the context of embryonic development.
%In the future, we plan to study embryonic development, and in general the evolution of hierarchical 
%modular networks in an optimization framework. Such an approach can provide 
%more direct insight into the processes that shape the evolution and structure of these networks.


==> tex_files/embryonic_development/embryonic_development.tex <==
\section{Embryonic Development} \label{sec:embryo}

% Describe embryonic development in general, 
% Introduce the spatoi-temporal progression of development at the genomic level,
% Introduce the concept of a temporal gene dependency network (TGDN)
% Introduce the concept of increasing specifity.
% Introduce the evolutionary changes that can occur in a TGDN
% In this section, we do not get into the details of how we model each of these observations. Rather we just state the facts.


If we do not consider the external effects on the cells of the developing embryo,
the state of a gene in time and space can be traced back to the 
initial configuration of the developmental GRN, i.e.
the states of the maternal genes.
The execution of the genomic program can then be viewed as a layered directed acyclic graph (DAG) 
of active regulatory gene interactions as they unfold 
over time and space as illustrated in Figure \ref{fig:embryo}-a.
These regulatory interactions are accomplished (or activated) either 
through encoding (or not encoding) transcription factors
or signaling molecules.
Each layer of the graph corresponds to a developmental stage and includes 
the genes that are active at that stage. Inactive genes in 
a certain stage of the development are left out
because {\em their regulatory states stays constant and so no new information
flows through these genes from the previous stage to the next.}
We refer to this graph as the {\em temporal gene dependency network} or {\em TGDN}.

The evolutionary aspect of embryonic development includes the mechanisms that 
modify the structure of the genes and the GRN that participate in the development, as well as the 
associated natural selection process.
The evolutionary mechanisms and their effect on the developmental TGDN are illustrated in Figure \ref{fig:embryo}-c.
These mechanism include deleterious mutations (DM), mutation that change the 
function of a gene (NM), and gene duplication (GD). Mutations
can also lead to {\em gene regulatory failure (RF)} and {\em developmental failure (DF)} for the organism.
Regulatory failure happens when a gene loses some of its regulators 
and cannot become active at the right stage of the development.
Developmetal failure happens when some of the genes belonging to the last stage of development fail to regulate correctly.
Most of those genes belong to {\em developmental gene batteries}\footnote{Sets of related
genes that are expressed in unison.} that express tissue-specific proteins.
Their mis-regulation can lead to lethal birth defects for the organism.


==> tex_files/modeling_variations.tex <==
%\vspace{-10pt}

%\section{Location of the waist}
\noindent {\bf Location of the waist}\\
We examine here two parameters of the model that can be used to control the 
location of the waist in the DGDNs that result from evolution.

The first parameter is the stage specificity function which affects how NM events act on genes.
To examine its effect, we make use of a sigmoid 
function where we can vary the stage with the specificity of $50\%$ (See SI-Fig. \ref{fig:sigmoid_specificity}). We 
denote this stage by $\gamma$. This is the stage with maximum
variability for a gene's downstream regulators
and so NM events on genes cause the largest rewiring in 
the set of such genes and potentially several RFs. 
As a result, by varying $\gamma$ along the internal stages of the DGDN, we observe that  
the waist of the hourglass tends to form close to stage $\gamma$ (See SI-Fig. \ref{fig:waist_location}-a).
The second parameter is the RF parameter $z$ which controls the RF probability. 
Increase in $z$ leads to a decrease in 
the rate of evolutionary changes due to NM events in DGDNs 
of the surviving individuals--most of such events end up causing 
lethal RF cascades for the organism. Such lethal RF cascades become 
more likely when a gene has a large number of downstream regulators, i.e. 
as we move upstream in the DGDNs. This is because removal of a gene can potentially affect 
several downstream genes and lead to a lethal cascade for the individual (due to large probability 
of RF). As a result, by increasing $z$ we observe 
that the waist of the hourglass moves downstream in the 
DGDNs (See SI-Fig. \ref{fig:waist_location}-b).\\

%\vspace{-10pt}
%\section{Regulatory gene rewiring}
\noindent {\bf Regulatory gene rewiring}\\
We have also examined how the NM mechanism affects the structure of 
the resulting DGDNs. To do so we considered two variations. 
In one variation we examine the case where upstream regulators 
are rewired similar to downstream regulators (rather than 
chosen from scratch). 
%Fig. \ref{fig:other_results}-c shows the median normalized outdegree of the genes 
%of each stage (together with the 10th and 90th percentiles). 
In this case, while loss of downstream regulators due to NM events can lead 
to lethal RF cascade events and the 
removal of the individual from the population, gain of such regulators 
does not have the same effect.
The DGDNs become denser over time as a result. This result can be viewed
as unrealistic because gene regulation is costly specially intercellular 
signaling and regulation across different domains of the embryo.
In a second variation, we examined the case where both upstream 
and downstream regulators are chosen from scratch 
based on the specificity of the corresponding stages. 
%Fig. \label{fig:other_results}-c shows the age of the genes with this NM variation. 
In this case as we move downstream in a 
DGDN, it becomes more likely that 
an NM event will lead to major rewiring in the downstream 
regulators of the gene. These rewiring 
can lead to lethal cascade events. As a result, the hourglass shape disappears from 
the age of the genes and an increasing 
trend (for $l=1..9$) emerges instead. This result is not in agreement with previous empirical
observations \cite{domazet2010phylogenetically}.

Based on our model and the analysis in this section, we expect an NM event to 
have two main properties when it acts on genes: 1) it causes the most lethal 
perturbation in the DGDN when it occurs near the waist, and 2) it preserves the 
overall normalized degree distribution of the stage. We can speculate that the former is due to
the highly constrained nature of the genes close to the waist as also supported 
by our results on the age and prevalence of genes as well as previous studies \cite{}.
The latter is an structural constraint of the developing embryo imposed by the 
gradual formation and separation of distinct domains which increase the cost of intracellular
signaling and regulation. In theory and within the context of our model, 
any abstract NM mechanism that preserves these properties
could be a plausible candidate to capture mutations that lead to new functionalities in the genome.\\

%\vspace{-20pt}


==> tex_files/models/devo_model.tex <==
\subsection{Model of the developmental process}

Even though every cell of the developing embryo carries the same genome,
different cells are in different {\em regulatory states}.
during the developmental process,
depending on the cell's lineage as well as on the set of transcription factors, 
maternal mRNA and other transduction signals that are active in the nucleus of each cell.
As development progresses and the various spatial domains of the embryo gradualy take shape, 
the expression level of some of the genes can go through significant changes in each cell of the embryo. 
The collection of expression levels 
of all the gene in a cell can determine the regulatory state of that cell at any point during development.
In the following, we describe how in particular we model embryonic development at the genomic level in more detail. 
We first describe how a gene's expression level can be translated to a {\em functional state}.
We then describe that the developmental process can be modeled as the execution of the genomic program, i.e., the
progression of gene functional states which unfold differently at each part of the developing embryo.
Note that we make several abstractions of the underlying biological mechanisms to provide a minimal
yet realistic model of embryonic development at the genomic level.\\

{\bf Gene functional state (FS)}: 
A regulatory gene can be in one of 
two (or in general several) {\em functional states (FS)} 
in any cell of a living organism at any point in time. 
Each state corresponds to an expression level of the gene in the cell nucleus.
A gene in this view is encoding a {\em bit} of information and is binary in nature as 
in a classical digital computing system. The gene can either be expressed (ON) or repressed (OFF). 
In a more general context, genes can have several expression states, i.e., be in a 
superposition of both ON and OFF states at the same time similar to a qubit in the quantum computing context.
The expression level (or state) of a gene at 
a certain time during development is a function (boolean or analogue depending on the view)
of the expression level (or state) of it regulators.
For the simplicity of description, in the rest of this paper, we refer to 
a gene as being either in the OFF or ON states.\\

{\bf Functional state (FS) transition:}
When a gene changes its functional state, i.e. in a binary context when it is down-regulated to turns OFF
or up-regulated to turn ON,
the gene goes through a {\em functional state (FS) transition}.
A gene's FS or in general expression level depends 
on the FS of its regulators. This information is encoded 
in the organism's developmental gene regulatory network (GRN) which specifies the 
exact logical function that gives the FS of each gene based on the 
FS of its regulators. In our model, we make the assumption that a gene's FS 
is controlled only by encoding (or lack of encoding) 
of transcription factors or signaling molecule. Based on this assumption,
FS transitions in the regulators of a gene can trigger FS transition 
in the gene itself.

The genomic program that is executed during development can then be viewed as 
the {\em spatio-temporal cascade} of FS transitions which unfolds differently at different 
domains of the developing embryo. Each FS transition is triggered (or regulated) 
by one or more FS transitions that 
precede it. A failing row of dominoes can be used as an analogy to the 
execution of this genomic program.
The program is initialized with the FS of the maternal 
genes in the zygote as inputs to the developmental GRN. The FS 
of these genes is controlled by maternal mRNA and other
external signals. The execution then proceeds in a semi-autonomous fashion 
with the configuration of maternal regulatory genes as its initial state.
We model the cascade of FS transitions as a network of gene dependencies which we refer to as a
{\em temporal gene dependency network (TGDN)}. We define TGDN below.\\

{\bf Temporal gene dependency network (TGDN):} 
A TGDN captures the progression of the genomic program in $L$
discrete-time snapshots or {\em stages} of development. 
The duration of each stage, in terms of absolute time, does not need to be
the same across all stages; different regulatory interactions proceed at different rates.
Any stage $1< l < L$ includes a gene that meet the following criteria:

1. The gene goes through an FS transition at that stage of the 
development in at least one spatial domain of the embryo. 

2. The gene affects the FS transition of at least one gene in the next stage of the development.

The genes at the first stage ($l=1$) are, by convention, any maternal regulatory gene that 
satisfies the second citeria above. Additionally, we do not model the developmental process beyond 
stage $L$ and the genes at the last stage ($l=L$) should only satisfy the first criteria.
Those genes are either very tissue specific and encode tissue specific proteins or 
regulate the expression of very tissue specific genes.


Together the genes at all stages consititute the nodes of the network. 
The set of genes at a stage $l=1,\dots L$ is denoted by $G(l)$.

A regulatory gene $g$ at stage $l<L$ of a TGDN participates in the developmental process by 
affecting (or regulating) the FS transition of a set of downstream regulatory genes $D(g)$ which
reside in the next developmental stage $l+1$. The set $D(g)$ essentially determines g's {\em function} 
at that stage of the TGDN.
Similarly, a gene $g$ at stage $l>1$ depends on the FS transition of
a set of {\em upstream} regulatory genes $U(g)$ in stage $l-1$.
These FS transition dependencies constitute the links of the network.

The set of genes in all $L$ stages which constitue the TGDN is denoted by $G$. 
Note that the TGDN does not capture the exact ``input function''
for each gene (e.g., whether it is a Boolean or an analogue function of the 
expression level of the gene's regulators), and it does not treat differently 
regulatory genes that act as promoters or repressors. 
Further, because GRNs contain feedback loops and so a gene may change functional
state more than once during development, the TGDN may include a certain
gene in more than a single stage. 
A TGDN essentially is a {\em static representation} of a dynamic process, i.e. the 
unfolding of FS transition cascades at different spatial domains of the embryo.
Figure \ref{fig:embryo}-a shows a TGDN.


As the various spatial domains of the embryo gradually take shape, 
increasingly more tissue-specific genes go through FS transitions.
The genes become more specific to the spatial domain, i.e., the body part, they are active in. 
On the other hand, the ever-growing distance between distinct spatial domains,
increases the cost of intercellular signaling across different domains. As a result,
the likelihood of cross-domain regulation decreases as development progresses. 
This effect is captured by assigning a {\em functional specificity'' to each developmental stage} which
is defined below.\\


{\bf Stage functional specificty:}
The functional specificity of a stage $l$ of a TGDN determines the likelihood 
of the {\em absence} of a link between genes of stage $l$ and $l+1$.
Figure \ref{fig:embryo}-b shows two examples of how 
the {\em functional specificity} of developmental stages increases over time. We later show that 
this increasing specificity assumption is required for our models to produce the 
biological observations.


==> tex_files/models/evo_model.tex <==
\subsection{Model of Evolutionary Process}
We consider a population of individuals that, at least initially,
all have the same TGDNs and belong to the same species.
We assume that the individuals reproduce asexually in each generation,
and the number of individuals in the population remains constant.

Here we describe how we model the several evolutionary mechanisms that modify the 
structure of a TGDN. We consider three evolutionary changes that act on genes: 
1) Neomorphic mutations 2) Deleterious mutations 3) Gene duplication.
We also describe how these changes affect the activation of genes 
in the TGDN and the survival of the individual.\\

{\bf Gene duplication (GD):} A gene $g$ can get duplicated and
an identical copy of the gene with the same exact $D(g)$ and $U(g)$ 
will be created at the same stage as the duplicated gene. 
The two genes will stay identical until at least one of them goes 
through a neomorphic mutation, or one is removed due to deleterious mutation.
A gene can be duplicated at each generation with probability $P_{GD}$.\\


{\bf Neomorphic mutations (NM): } This mutation captures the 
gradual changes in the function of a gene (i.e. $D(g)$) 
as well as its set of regulators (i.e. $U(g)$) that can 
accumulate over evolutionary timescales and result in a neomorphic gene.
Through this event, some of the gene's upstream and 
downstream regulatory links can get rewired and change. 
Specifically considering a gene $g$ at stage $l$, first the set $U(g)$
is determined from scratch based on the specifity of the previous stage (i.e. $1 - s(l-1)$).
Then we proceed to determine the gene's new function, i.e., its new $D(g)$. 
To do so, we find the number of downstream 
links that the gene will lose as a binomial random variable 
$\beta=B(|D(g)|, 1 - s(l))$ and the number of new downstream links that 
the gene will gain as another binomial random variable 
$\alpha=B(|D(g)|, 1 - s(l))$. We then randomly choose and remove $\beta$
unique genes (together with their duplicates if any) from $D(g)$ and add $\alpha$ 
new unique genes (together with their duplicates if any) to $D(g)$. Note that the mutation 
event may change the number of downstream regulatory genes (i.e. $|D(g)|$) of gene $g$.
The use of specificity 
captures the fact that the higher a gene resides in the TGDN (i.e. as development progresses),
the more tissue specific it becomes and so its functionality 
would be more constrained and localized to the specific spatial domain the gene is active in 
and so is less likely to change significantly through mutations. 
Note that duplicate genes will stay identical in terms of their upstream and downstream 
regulators until one of them experiences a GD event 
in which case the duplicates start to diverge from each other.
Figure \ref{fig:embryo}-c illustrates how the mutation event acts on a gene.
A gene can go through neomorphic mutation at each generation with probability $P_{NM}$.\\

{\bf Deleterious mutations (DM): } This type of mutation occurs when the genomic sequence of a 
gene is altered in such a way that it becomes disfunctional. The gene in this case can be considered 
in the OFF state all the time and so cannot go through FS transitions at any stage of development. 
By definition, this gene is removed from the TGDN together with all of its (previously) active regulatory links.
A gene can go through deleterious mutation at each generation with probability $P_{DM}$.\\ 

{\bf Regulatory failures (RF)}:  
Mutations in a gene can cause ``regulatory failures'' 
in the set of its downstream regulatory genes.
Note that in this definition, a regulatory failure in a gene does 
not mean that the gene will turn OFF but rather it means that the gene will fail to correctly 
go through an FS transition at the right stage of development.
The idea of regulatory failure comes from the nested canalyzing boolean rules
introduced by Kauffman \cite{Kauffman} which appear in the context of random boolean genetic networks. 
{\em ({\bf NOTE: Information dump from Kauffman papers here}) A canalyzing rule is a Boolean rule with the property that one
of its inputs alone can determine the output value, for either
``true'' or ``false'' input. This input value is referred to as the
canalyzing value, the output value is the canalyzed value, and we
refer to the rule as being canalyzing on this particular input. 
Nested canalyzing rules are a very natural subset of canalyzing
rules, stemming from the question of what happens in the noncanalyzing
case, that is, when the rule does not get the canalyzing
value as input but instead has to consult its other inputs. If the rule
then is canalyzing on one of the remaining inputs and again for that
input’s noncanalyzing value, and so on for all inputs, we call the rule
nested canalyzing \cite{Kauffman}.}
In our model, we do not capture the exact boolean function on the set of upstream regulatory 
genes $U(g)$ that could determine the FS of gene $g$ at any point in time.
However, a nested canalyzing rule means that the FS transition of gene $g$ at stage $l$,
would depend on the correct FS transitions of at least a subset of genes in $U(g)$. 
So the more a regulatory gene $g$ loses its upstream regulators, possibly due to NM or DM events in those genes, 
the more likely it is to fail to go through state transition correctly.
The function to determine when a gene experiences a regulatory failure is captured based on the number 
of the gene's upstream regulators. With this function we also try to capture 
the notion of biological redundancy and the fact that 
the up-regulation or down-regulation of a gene 
may be successful even if some of its regulators are "broken".
Mathematically, a gene $g$ is more likely to experience a 
regulatory failure if it loses a large fraction of its unique downstream regulators due to the mutation event.
Considering a gene $g$ , if we denote the set of $g$'s unique regulators before the start of the 
mutation by $U^{'}(g)$ and its current set of unique regulator by $U(g)$, then if
$|U(g)|<|U^{'}(g)|$, the gene is removed with probability :
\begin{align}
p_d(r)=1-e^{\frac{-z_{RF} \, r}{1-r}},\\
\mbox{where } r=1-\frac{|U(g)|}{|U^{'}(g)|}\notag
\end{align}

A mutation in a gene can lead to a cascede of regulatory failure as depicted in Figure \ref{fig:embryo}-c
which originate at the mutated gene. In such cases, 
the failure in the FS transition in one gene can have a cascade effect over developmental time 
and lead to several subsequent failures in the downstream genes and potentially at several spatial domains.
This can potentially lead to {\em developmental failure} in the organims.\\

%The {\em regulatory failure probability function} $p_d(r)$ is shown in Figure~\ref{fig:rf}
%for three different values of the {\em regulatory failure parameter} $z_{RF}$.\\


%\begin{figure}[!htb]
%\centering
%    \includegraphics[width=50mm,height=95mm,angle=270]{figures/deathFunction.eps}
%    \caption{The death probability for three values of the regulatory failure
%parameter $z$.}
%    \label{fig:rf}
%\end{figure}

{\bf Developmental failure (DF) and natural selection:}
Developmetal failure happens when some of the genes belonging to 
the last stage of development fail to go through FS transitions correctly.
Most of those genes belong to {\em developmental gene batteries}\footnote{Sets of related
genes that are expressed in unison.} that express tissue-specific proteins.
Their mis-regulation can lead to lethal birth defects for the organism.
We capture developmental failures 
based on the number of genes at stage $L$ of the TGDN with respect 
to a target number of genes denoted by $\Gamma$. Such developmental failures
can happen either due to deleterious mutations (DMs) or regulatory failures (RFs)
in the genes of the last stage. In the simplest case, if the
 number of those genes, $|G(L)|$ drops below $\Gamma$ then the individual would die
and be replaced randomly with an individual that survives
the developmental process in the same generation (i.e., the population size remains
constant as long as at least one individual survives).


==> tex_files/models/model_description.tex <==
\section {Model Description} \label{sec:model_desc}

% Functional state transition
% TGDN (static view of a dynamic process)
% What are nodes in a TGDN?
% What are edges in a TGDN?
% What are the evolutionary mechanisms that can change a TGDN from one generation to the other
% What are the effects of the evolutionary changes on the individuals and their survival

We describe here our model of embryonic development and its evolution at the genomic level, considering
two different timescales. We first focus on the developmental time scale, i.e. from the 
time of conception and formation of the zygote to the time of birth, hatching, or germination 
depending on the type of the organism. Then we focus on the evolutionary timescales and describe 
how evolution alters the genetic structure of the organism and the processes involved in embryonic development.

Even though every cell of the developing embryo carries the same genome,
different genes in the cell can have different expression levels. The expression levels of the genes are 
controlled by {\em regulatory genes}, a subset of the genes that encode transcription factors or 
signaling molecules. 

Depending on its expression level, a regulatory gene can be 
in one of several {\em functional states}. Here, the expression level of a gene 
is assumed to come from a discrete set of values each corresponding to a functional 
state \cite{}. When a gene's expression level switches between its possible values,
the gene goes through a {\em functional state transition}. Such transitions are not 
instantaneous and can take place in variable speeds \cite{}.

%A regulatory gene can affect (or regulate) the expression of other genes in the cell of the embryo 
%by encoding transcription factors or signaling molecules. The production level of these 
%gene products is controlled by the gene's functional state.
The gene regulatory network (GRN) of an organism specifies the regulatory 
interactions that control the expression level of each gene of that organism 
as well as the functional relations that 
determine the functional state of each gene from its inputs. 
%The GRN however by itself does 
%not contain any explicit information regarding the functional 
%state of a gene at any point in developmental time and space. 
As development progresses, regulatory genes go through functional state transitions.
These transitions then unfold over time and space similar to a failing row of dominoes. 
Each transition depends on (or is triggered by) one or more transitions that precede it. 
The unfolding of these functional state transitions dependencies can then 
be captured in a network where nodes are genes that go through such transitions
and edges are gene regulatory dependencies.
We refer to this network as the developmental gene dependency network (DGDN).
Figure \ref{fig:embryo}-a shows a DGDN.
%Development can then be viewed as the execution of a genomic program. 
%This program is initialized with the functional states of the maternal 
%genes in the zygote which is plugged into the developmental GRN. 
%The functional state of these genes is controlled by maternal mRNA and other external signals. 
%The execution then proceeds in a semi-autonomous fashion 
%with the configuration of maternal regulatory genes as its initial state.

A DGDN captures the progression of development in $L$
discrete-time snapshots or {\em stages} of development. 
The duration of each stage, in terms of absolute time, does not need to be
the same across all stages. Furthermore, the total number of stages, i.e. the parameter $L$, is a developmental propoerty
and is chosen so that as many functional state transitions as possible are captured.
The set of genes at a stage $l=1,\dots L$ is denoted by $G(l)$.
A gene $g$ at stage $l$ regulates a set of {\em downstream} genes at stage $l+1$ denoted by $D(g)$. 
%The set of {\em downstream} regulatory genes that depend on a gene $g$ at stage $l<L$ is denoted by $D(g)$ and
%reside in the next developmental stage $l+1$. 
Similarly, a gene $g$ at stage $l>1$ is regulated by
a set of {\em upstream} regulatory genes $U(g)$ in stage $l-1$.

%Connecting paragraph
The goal of a DGDN is to capture 
the execution of a genomic program, i.e. the
sequence of functional state transition events as they unfold over time and the spatial domains of the embryo.
A DGDN however, does not capture the exact identity of each gene or the exact input function
that would determine the functional state of each gene, and it does not treat differently 
regulatory genes that act as promoters or repressors.
The model presented here focuses on the structure of a DGDN and how it
affects the success of the developmental process subject to evolutionary changes
that can occur in the genome of the organism witin a population of competing individuals.
 
Each developmental stage is assigned a {\em spcificity} denoted by $s(l)$ for 
stage $l$ of the DGDN and captures the 
density of the DGDN at that stage. $s(l)$ determines the likelihood 
of the {\em absence} of an edge from a node at stage $;$ to a node at stage $l+1$.
As the various spatial domains of the embryo gradually take shape, 
the genes of the DGDN
become more restricted to the spatial domain, i.e., the body part, they are active in. 
On the other hand, the ever-growing distance between distinct spatial domains,
increases the cost of intercellular signaling across different domains. As a result,
the likelihood of cross-domain regulation decreases as development progresses. 
As a result, {\em specificity} is an increasing function of 
the developmental stage (See Figure  \ref{fig:embryo}-b for sample specificty functions). 

The DGDN of an individual is subject to evolutionary changes which can modify its
structure.
In the following, we procedd to describe these evolutionary mechanisms. 
We consider three evolutionary changes that act on genes: 
1) Neomorphic mutations 2) Deleterious mutations 3) Gene duplication.
We also describe how these changes affect the correct functional state transitions of genes 
in the DGDN and ultimately the survival of the individual. Figure \ref{fig:embryo}-c
illustrates these mechanisms.\\

{\bf Gene duplication (GD):} A gene $g$ can get duplicated and
an identical copy of the gene with the same exact $D(g)$ and $U(g)$ 
will be created at the same stage as the duplicated gene. 
The two genes will stay identical until at least one of them goes 
through a neomorphic mutation, or one is removed due to deleterious mutation.
A gene can be duplicated at each generation with probability $p_{GD}$.\\

{\bf Neomorphic mutations (NM): } 
%This mutation captures the 
%gradual changes in the function of a gene (i.e. $D(g)$) 
%as well as its set of regulators (i.e. $U(g)$) that can 
%accumulate over evolutionary timescales and result in a neomorphic gene.
A neomorphic mutation captures how a gene's upstream and 
downstream regulatory edges can get rewired and change over time. 
Specifically considering a gene $g$ at stage $l$, first the set $U(g)$
is determined from scratch based on the specifity of the previous stage (i.e. $1 - s(l-1)$).
Then we proceed to determine the gene's new function, i.e., its new $D(g)$. 
To do so, we find the number of downstream 
links that the gene will lose as a binomial random variable 
$N_{-}=B(|D(g)|, 1 - s(l))$ and the number of new downstream links that 
the gene will gain as another binomial random variable 
$N_{+}=B(|D(g)|, 1 - s(l))$. We then randomly choose and remove $N_{-}$
unique genes (together with their duplicates if any) from $D(g)$ and add $N_{+}$ 
new unique genes (together with their duplicates if any) to $D(g)$. Note that the mutation 
event may change the number of downstream regulatory genes (i.e. $|D(g)|$) of gene $g$.
A gene can go through neomorphic mutation at each generation with probability $p_{NM}$\\

{\bf Deleterious mutations (DM): } This type of mutation occurs when the genomic sequence of a 
gene is altered in such a way that it becomes disfunctional. The gene 
cannot go through functional state transitions at any stage of development and so 
is removed from the DGDN together with all of its (previously) active regulatory edges.
A gene can go through deleterious mutation at each generation with probability $p_{DM}$.\\ 

{\bf Regulatory failures (RF)}:  
Mutations in a gene can cause ``regulatory failures (RF)'' 
in the set of its downstream regulatory genes.
An RF for a gene means that the gene will fail to correctly 
go through a functional state transition at the right stage of development.
With an RF we also try to capture 
the notion of biological redundancy and robustness of GRNs to random failures \cite{}-- 
that the up-regulation or down-regulation of a gene 
may be successful even if some of its regulator dependencies are ``broken''.
%However the more a regulatory gene $g$ loses its upstream regulators, possibly due to NM or DM events in those genes, 
%the more likely it is to fail to go through state transition correctly.
The function to determine when a gene experiences a regulatory failure is captured based on the number 
of the gene's upstream regulators. 
Mathematically, a gene $g$ is more likely to experience a 
regulatory failure if it loses a large fraction of its unique downstream regulators due to an evolutionary event.
Considering a gene $g$, if we denote the set of $g$'s unique regulators before the start of the 
event by $U(g)$ and its current set of unique regulator by $U_{new}(g)$, then if
$|U_{new}(g)|<|U(g)|$, the gene is removed with probability :
\begin{align}
p_d(r)=1-e^{\frac{-z_{RF} \, r}{1-r}},\\
\mbox{where } r=1-\frac{|U_{new}(g)|}{|U(g)|}\notag
\end{align}

Mutations in a gene can lead to a cascede of regulatory failure as depicted in Figure \ref{fig:embryo}-c
which originate at the mutated gene. In such cases, 
the failure in the functional state transition in one gene can have a cascade effect over several stages of the DGDN 
and lead to multiple subsequent failures in the downstream genes.
This can potentially lead to {\em developmental failure} in the organims.\\

{\bf Developmental failure (DF):}
The genes at the last stage of the DGDN control the 
final outcomes of the developmental process
and essentially determine the fate of the embryo.
The process may not be successful if some of the genes that encode 
tissue specific proteins are not expressed correctly at the end
(i.e., at the time of birth, hatching, or germination).
In our model, we simply capture these developmental failures 
based on the number of genes at stage $L$ of the DGDN with respect 
to a target number of genes denoted by $\Gamma$. If the
number of those genes, $|G(L)|$ drops below $\Gamma$ 
then the individual would die
and be replaced randomly with an individual that survives
the developmental process in the same generation (i.e., the population size remains
constant as long as at least one individual survives).\\

In this section, we presented an abstract model of embryonic development. The aim of this model is not 
to determine the exact expression pattern of every gene during development or 
the fate of every cell of the embryo. The model captures the structure of regulatory 
gene interactions as they unfold over time and space in the form of a network of gene dependencies.
It then focuses on how the structure of this network evolves over (evolutionary) 
time and how this structure affects the success of the embryonic development.

\subsection{Models}
To study the effect of the important mechanisms in our model we proceed as follows. We build three different 
models starting with a minimal model of embryonic development. 
We then gradually add new mechanisms and tune the parameters to make the model more complete. We study the 
behavior of each model with respect to the structure of the evolving DGDNs and some specific properties of the genes 
in the DGDNs.

\subsubsection{Model 1}
The model includes a population of $N=10$ identical 
individuals all having 100 genes 
at every stage of their DGDNs. 
The number of stage $L=10$.
$s(l)$ for $l=1..L$, i.e. the specificty of each stage, is the same and equal to 0.5.
The model advances in discrete-time steps or generations. 
At each generation, every individual's DGDN is checked starting from the erliest stage ($l=1$). The DGDNs
can then get modified through only NM events with probability $p_{NM}=10^{-4}$. 

\subsubsection{Model 2}
This model is identical to the previous model in terms of the mechanisms involved. The only differece is 
that $s(l)=l/L$, i.e., specificy is an increasing function of the stage number.

\subsubsection{Model 3}
This model is built on top of the previous model and includes duplictions as well. The duplication probability $p_{DM}$ is 
adjusted adaptively ($10^{-6}<p_{DM}<10^{-5}$)so that the average number of genes in each invididual stays within an upper and lower limit ($700<\hat{|G(l)|}<800$).


==> tex_files/models/model_exec.tex <==
\subsection{Model Execution}

The model execution starts with a population of identical 
individuals all having the same number of genes 
at each stage of their TGD networks. 
The model then advances in discrete-time steps or generations. 
In the most complete version of the model, at each generation, e
very individual's TGD network can get 
modified through duplications, mutations, and potential regulatory
failure cascades in dependent of other individuals. 
To do so every individuals TGD is examined in a bottom up manner starting from 
stage 1 going up to stage L. At every stage the following tasks are performed:

a) Check genes for NMs with probability $P_{NM}$, perform the rewiring and 
determine the new regulatory interactions.

b) If a unique gene gets mutated, determine the potential regulatory 
failure cascade that follows and whether the individual would die due 
to developmental failure.

c*) Check genes for $DM$ with probability $P_{DM}$.

d*) If a unique gene gets mutated, determine the potential regulatory 
failure cascade that follows and whether the individual would die due 
to developmental failure.

e*) Check genes for duplication with probability $P_{GD}$.

Once all the individuals have been checked, the dead ones will be replaced
by randomly chosen surviving individuals.

In the next following section, we slowly start adding the different components described here 
to a ``minimal'' model of embryonic development and observe how those different 
components affect the results of the model.

